Topological Field Theories and Harrison Homology

The tools and arguments developed by Kevin Costello are adapted to families of "Outer Spaces" or spaces of graphs. This allows us to prove a version of Deligne's conjecture: the Harrison homology associated to a homotopy commutative algebra is naturally a module over a particular cobordism category of 3-manifolds.

==> graphicx.tex <==
% Plain TeX interface to graphicx package.
% David Carlisle


%\input miniltx

%\def\Gin@driver{dvips.def}
%\input graphicx.sty


%\resetatcatcode

\input miniltx

\ifx\pdfoutput\undefined
  \def\Gin@driver{dvips.def} % we are not running PDFTeX
\else
  \def\Gin@driver{pdftex.def} % we are running PDFTeX
\fi
 
\input graphicx.sty
\resetatcatcode

